Resolution of the Co-Location Problem in Satellite Quantum Tests of the Universality of Free Fall

A major challenge common to all Galilean drop tests of the Universality of Free Fall (UFF) is the required control over the initial kinematics of the two test masses upon release due to coupling to gravity gradients and rotations. In this work, we present a two-fold mitigation strategy to significantly alleviate the source preparation requirements in space-borne quantum tests of the UFF, using a compensation mechanism together with signal demodulation. To this end, we propose a scheme to reduce the gravity-gradient-induced uncertainties in an atom-interferometric experiment in a dedicated satellite mission and assess the experimental feasibility. We find that with moderate parameters, the requirements on the initial kinematics of the two masses can be relaxed by five orders of magnitude. This does not only imply a significantly reduced mission time but also allows to reduce the differential acceleration uncertainty caused by co-location imperfections below the $10^{-18}$ level.

==> figs_and_tabs/phasetable.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|cc|cc}
    &\multicolumn{2}{l|}{no compensation} & \multicolumn{2}{l}{without compensation}\\
    \hline 
    
 1  & $\frac{1}{4} \delta v_{z,0} T \gamma \left(3 \cos (2 \chi )+1\right)$ 
    & $4.45\times10^{-12}$ 
    & $-\frac{2 \delta \theta \delta v_{x,0}}{T}$ 
    & $1\times 10^{-14}$\\
    
2   & $\frac{1}{4} \delta z_0 \gamma \left(3 \cos (2 \chi )+1\right)$
    & $2.23\times 10^{-12}$
    & $\frac{2 \delta \theta  \delta v_{x,0}}{T}$ 
    & $1\times 10^{-14}$\\
    
3   & $\frac{3}{4} \delta x_0 \gamma T \Oo \cos (2 \chi )$
    & $3.53\times 10^{-14}$
    & $-\frac{2 \delta \theta  \delta x_{0}}{T^2}$ 
    & $5\times 10^{-15}$
    
4   & $\frac{1}{4} \delta v_{x,0} \gamma T^2 \Oo \cos (2 \chi )$
    & $2.35\times 10^{-14}$
    & $\frac{\delta \theta  \delta x_{0}}{T^2}$ 
    & $5\times 10^{-15}$


\end{tabular}
\end{table}




%\begin{comment}
% 2 & \frac{1}{4} \text{$\delta $z0} \text{Tzz0} (3 \cos (2 \chi )+1) & \text{2.227302327114841$\grave{ }$*${}^{\wedge}$-12} & \frac{2 \delta
%   \theta  \text{$\delta $vx0}}{T} & \text{1.0000000000000002$\grave{ }$*${}^{\wedge}$-14} \\
% 3 & \frac{3}{4} \text{$\delta $x0} T \text{Tzz0} \text{$\Omega $orbit} \cos (2 \chi ) & \text{3.525697254545301$\grave{ }$*${}^{\wedge}$-14} &
%   -\frac{2 \delta \theta  \text{$\delta $x0}}{T^2} & \text{5.$\grave{ }$*${}^{\wedge}$-15} \\
 %4 & \frac{1}{4} \text{$\delta $vx0} T^2 \text{Tzz0} \text{$\Omega $orbit} \cos (2 \chi ) & \text{2.3504648363635343$\grave{
%   }$*${}^{\wedge}$-14} & \frac{\delta \theta  \text{$\delta $x0}}{T^2} & \text{2.5$\grave{ }$*${}^{\wedge}$-15} \\
 %5 & 2 \text{$\delta $vx0} \delta \Omega  & \text{9.999999999999999$\grave{ }$*${}^{\wedge}$-16} & 2 \text{$\delta $vx0} \delta \Omega  &
 %  \text{9.999999999999999$\grave{ }$*${}^{\wedge}$-16} \\
% 6 & -2 \text{$\delta $vy0} \delta \Omega  & \text{9.999999999999999$\grave{ }$*${}^{\wedge}$-16} & -2 \text{$\delta $vy0} \delta \Omega  &
 %  \text{9.999999999999999$\grave{ }$*${}^{\wedge}$-16} \\
 %7 & \frac{5}{96} \text{$\delta $z0} T^2 \text{Tzz0}^2 (3 \cos (2 \chi )+5) & \text{8.268126093951978$\grave{ }$*${}^{\wedge}$-16} & \frac{1}{4}
 %  \text{$\delta $Tzz0} \text{$\delta $vz0} T (3 \cos (2 \chi )+1) & \text{2.$\grave{ }$*${}^{\wedge}$-16} \\
%8 & \frac{1}{96} \text{$\delta $vz0} T^3 \text{Tzz0}^2 (3 \cos (2 \chi )+5) & \text{3.3072504375807913$\grave{ }$*${}^{\wedge}$-16} &
   %\frac{1}{4} \text{$\delta $Tzz0} \text{$\delta $z0} (3 \cos (2 \chi )+1) & \text{1.$\grave{ }$*${}^{\wedge}$-16} \\
 %9 & \frac{1}{4} \text{$\delta $Tzz0} \text{$\delta $vz0} T (3 \cos (2 \chi )+1) & \text{2.$\grave{ }$*${}^{\wedge}$-16} & -\frac{2
   %\text{$\delta \Delta $f} \text{$\delta $vz0}}{f T} & \text{1.$\grave{ }$*${}^{\wedge}$-17} \\
 %10 & \frac{1}{4} \text{$\delta $Tzz0} \text{$\delta $z0} (3 \cos (2 \chi )+1) & \text{1.$\grave{ }$*${}^{\wedge}$-16} & \frac{2 \text{$\delta
  % \Delta $f} \text{$\delta $vz0}}{f T} & \text{1.$\grave{ }$*${}^{\wedge}$-17} \end{comment}
